SpeechGen: Unlocking the Generative Power of Speech Language Models with Prompts

Large language models (LLMs) have gained considerable attention for Artificial Intelligence Generated Content (AIGC), particularly with the emergence of ChatGPT. However, the direct adaptation of continuous speech to LLMs that process discrete tokens remains an unsolved challenge, hindering the application of LLMs for speech generation. The advanced speech LMs are in the corner, as that speech signals encapsulate a wealth of information, including speaker and emotion, beyond textual data alone. Prompt tuning has demonstrated notable gains in parameter efficiency and competitive performance on some speech classification tasks. However, the extent to which prompts can effectively elicit generation tasks from speech LMs remains an open question. In this paper, we present pioneering research that explores the application of prompt tuning to stimulate speech LMs for various generation tasks, within a unified framework called SpeechGen, with around 10M trainable parameters. The proposed unified framework holds great promise for efficiency and effectiveness, particularly with the imminent arrival of advanced speech LMs, which will significantly enhance the capabilities of the framework. The code and demos of SpeechGen will be available on the project website: \url{https://ga642381.github.io/SpeechPrompt/speechgen}

==> related_works_remove_.tex <==
\section{related works}
% \subsection{Textless NLP}
% Self-supervised speech representation learning has revolutionized the field of speech processing by enabling unsupervised learning from vast amounts of unlabeled speech data. It has demonstrated remarkable performance across a range of tasks, including automatic speech recognition (ASR), speech translation, voice conversion, and more.

% The improved quality of speech tokens obtained through the discretization of self-supervised speech representations has created new opportunities in the field of speech processing.

% Specifically, the Textless NLP project leverages these high-quality discrete speech tokens to apply natural language processing (NLP) techniques to speech-related tasks. One notable application is generative spoken language modeling\cite{, where NLP techniques are utilized to generate coherent and contextually relevant speech utterances.

% Moreover, discrete speech units have proven to be valuable in direct speech translation tasks. Specifically, pre-trained models such as the multilingual unit BART, which are trained on discrete speech units, have been successfully utilized in this domain.

% It is worth noting that speech language models in Textless NLP projects do not rely on text supervision during pre-training, distinguishing them from recent works that combine speech and text modalities within a single language model.

% Furthermore, the emergence of Textless NLP approaches has created opportunities to explore unwritten languages and facilitate communication in situations where written language may be limited or absent. These advancements hold great potential for preserving and understanding oral traditions, as well as addressing communication challenges in diverse linguistic contexts.

\subsection{Speech Language Models}
% Self-supervised speech representation learning has revolutionized the field of speech processing by enabling unsupervised learning from vast amounts of unlabeled speech data.
% The improved quality of speech tokens obtained through the discretization of self-supervised speech representations has created new opportunities in the field of speech processing.
Self-supervised speech representation learning \cite{mohamed2022self} has brought about a revolution in the field of speech processing by facilitating unsupervised learning from large volumes of unlabeled speech data.
By utilizing these self-supervised speech features, it has demonstrated remarkable performance across a wide range of downstream speech processing tasks \cite{DBLP:conf/interspeech/YangCCLLLLSCLHT21, DBLP:conf/acl/TsaiCHHLYDLLSCH22, DBLP:conf/slt/FengDYYLSCHWCWMLL22, wang2023minisuperb}
.
% Moreover, these self-supervised learning models can effectively tokenize and discretize high-quality speech tokens from continuous speech, opening up new avenues in speech processing for utilizing discrete speech tokens for speech language modeling.
Furthermore, by discretizing these self-supervised speech representations, it becomes possible to generate high-quality speech tokens directly from continuous speech. This advancement creates new possibilities in speech processing, enabling the utilization of discrete speech tokens for spoken language modeling~\cite{lakhotia2021generative}.


% Speech language models built on top of these enhanced speech units have shown remarkable capabilities. Utilizing generative language modeling techniques, GSLM, pGSLM, and AudioLM models have demonstrated the ability to generate novel speech, both conditionally and unconditionally. 
% Additionally, dGSLM is capable of generating natural spoken dialogues with spontaneous behaviors. Furthermore, Unit BART models have been employed in direct speech-to-speech translation tasks. 
% It is worth noting that these models are pre-trained on speech tokens without any text supervision.
% Speech language models built upon these enhanced speech units have exhibited remarkable capabilities.
% Generative Spoken Language Model (GSLM)~\cite{lakhotia2021generative}, prosody-aware Generative Spoken Language Model (pGSLM)~\cite{DBLP:conf/acl/KharitonovLPACL22}, Unit mBart \cite{popuri2022enhanced} has emerged as notable speech language models in the field, signaling the imminent development of advanced speech language models.
% GSLM specializes in performing language modeling on discrete units that encode phonetic information extracted by Hubert \cite{DBLP:journals/taslp/HsuBTLSM21}, a SSL (Self-Supervised Learning) speech model. 
% Building upon GLSM, pGSLM enhances the model's capabilities by incorporating prosody and duration in speech generation. 
% Additionally, Unit mBART extends the scope of speech language modeling to encompass multi-lingual scenarios, facilitating the generation of speech across different languages.
% It is worthy noting that these models are pre-trained on speech tokens without any text supervision.

Speech language models built upon these speech tokens have exhibited remarkable capabilities.
Generative Spoken Language Model (GSLM)~\cite{lakhotia2021generative}, prosody-aware Generative Spoken Language Model (pGSLM)~\cite{DBLP:conf/acl/KharitonovLPACL22}, and Unit mBart \cite{popuri2022enhanced} have emerged as notable speech language models in the field, signaling the imminent development of advanced speech language models.
GSLM specializes in performing language modeling on discrete units that encode phonetic information extracted by self-supervised speech models such as CPC, wav2vec2, and HuBERT. 
Building upon GSSM, pGSLM enhances the model's capabilities by incorporating prosody information spoken language modeling. 
Additionally, Unit mBART extends the scope of speech language modeling to encompass multi-lingual scenarios, facilitating the generation of speech across different languages.
It is worthy noting that these models are pre-trained on speech tokens without any text supervision.


% In addition to the "textless" speech language models, there are also models that incorporate text to enhance the generation expressiveness. Models like VALL-E and Spear-TTS perform text-to-speech (TTS) in a generative language modeling manner based on neural codes, such as soundstream and Encodec.
In addition to the ``textless" speech language models, there exist models that incorporate text to enhance the generation expressiveness. Models like VALL-E and Spear-TTS perform text-to-speech (TTS) in a generative language modeling manner based on neural codes, such as soundstream and Encodec.

% For the purposes of this paper, our focus is primarily on speech language models pre-trained without text supervision. This emphasis is due to the potential they offer in exploring unwritten languages and facilitating communication in situations where written language may be limited or absent. These advancements hold great promise for preserving and understanding oral traditions, as well as addressing communication challenges in diverse linguistic contexts.
In this paper, our primary focus lies on speech language models that conduct pre-training without text supervision.
The reason for this emphasis stems from that textless speech generation is of great significance, given the challenges posed by acquiring labeled text-speech pairs and the absence of text in certain languages.

\subsection{Prompting Speech Models}
% The prompting paradigm has experienced a surge in popularity since the launch of GPT-3. Its effectiveness stems from the ability to empower pre-trained language models, enabling them to efficiently handle a diverse range of tasks in a parameter-efficient manner, all within a unified feedforward process. By prepending the input with prompts that serve as task instructions, the model becomes proficient in effectively managing multiple tasks within the same batch. This distinction sets prompting apart from conventional model tuning and adapter tuning approaches, providing notable efficiency advantages for deploying models. 
The prompting paradigm has gained significant popularity, particularly with the introduction of GPT-3. 
This approach empowers pre-trained language models by leveraging prompts, which serve as task instructions, allowing the models to handle various tasks efficiently and in a parameter-efficient manner. 
Unlike traditional model tuning approaches, prompting utilizes a unified feedforward process and enables an LM to perform multiple tasks within the same batch \cite{DBLP:conf/emnlp/LesterAC21}. 
This unique feature provides significant efficiency advantages when deploying models \cite{DBLP:conf/icml/SunSQHQ22}.

In speech processing, SpeechPrompt \cite{DBLP:conf/interspeech/ChangT0L22} was a pioneering work that introduced prompt tuning based on GSLM, enabling it to excel in speech classification tasks such as keyword spotting and intent classification, as well as speech decoding tasks like ASR and slot filling. 
It demonstrated the effectiveness of prompting a speech language model to successfully handle a wide range of speech processing tasks.
% Further more, SpeechPrompt v2 explores the transferability of the prompting technique across different speech language models, specifically GSLM and pGSLM. 
% It investiaged the effectiveness of prompt tuning in facilitating more speech classification tasks, including multilingual and prosody-related aspects.
Furthermore, in SpeechPrompt v2 \cite{DBLP:journals/corr/abs-2303-00733}, the transferability of the prompting technique is investigated across different speech language models, specifically from GSLM to pGSLM. 
The study examines the effectiveness of prompt tuning in facilitating a broader range of speech classification tasks, including those involving multilingual and prosody-related aspects.
However, the effectiveness of prompts in eliciting generation tasks from speech language models still remains as an open question.
